Impact of Aviation Electrification on Airports: Flight Scheduling and Charging

Electrification can help to reduce the carbon footprint of aviation. The transition away from jet fuel-powered conventional airplane towards battery-powered electrified aircraft will impose extra charging requirements on airports. In this paper, we first quantify the increase in energy demands at several airports across the United States (US), when commercial airline carriers partially deploy hybrid electric aircraft (HEA). We then illustrate that smart charging and minor modifications to flight schedules can substantially reduce peak power demands, and in turn the needs for grid infrastructure upgrade. Motivated by our data analysis, we then formulate an optimization problem for slot allocation that incorporates HEA charging considerations. This problem jointly decides flight schedules and charging profiles to manage airport congestion and peak power demands. We illustrate the efficacy of our formulation through a case study on the John F. Kennedy International Airport.

==> figure/calculation.tex <==
%!TEX root = elsarticle.tex
\section{Calculation}
\label{sec:calculation}

To illustrate the power demand requirements through an example, consider a single hybrid electric retrofit of Embraer ERJ 170-200 aircraft with tail number N178SY operating a 599 miles flight from SFO to SLC (Salt Lake City, UT) on 05/29/2018. 
N178SY arrives at SFO at 17:02 PM and leaves for SLC at 17:53 PM. For different MF and BSED configurations, we compute $E$ from \eqref{eq:E.def} and report in Table \ref{tab:OneFlight}. Dividing $E$ by 60 minutes yields the power requirements of N178SY from  17:02 to  17:53 PM on 05/29/2018. Also note that this example illustrate the case where a hybrid electric aircraft does not have the range ability to cover a flight mission of distance 599 miles under the setting of BSED being 500 Wh/kg and MF being 25\%.

\begin{table}[!ht]
\centering
\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{MF (\%)}  & \multicolumn{2}{c}{BSED (Wh/kg)} \\\cmidrule(lr{1em}){2-3}
 &500 & 700 \\
\midrule
12.5  & 1.23 MW & 1.22 MW \\
25  & / & 2.52 MW \\
\bottomrule
\end{tabular}
\caption {Power requirements of N178SY for flight from SFO to SLC.} 
\label{tab:OneFlight} 
\end{table}


\begin{figure}[!h]
    \centering
    %---------
    \subfloat[MF=12.5\%, BSED=500Wh/kg]{\includegraphics[width=0.33\textwidth]{elsarticle/figure/dailyORD500.jpg}\label{fig:Daily:1}}
  \subfloat[MF=12.5\%, BSED=700Wh/kg]{\includegraphics[width=0.33\textwidth]{elsarticle/figure/dailyORD700.jpg}\label{fig:Daily:3}}
  \subfloat[MF=12.5\%, BSED=1000Wh/kg]{\includegraphics[width=0.33\textwidth]{elsarticle/figure/dailyORD1000.jpg}\label{fig:Daily:7}}
  %\captionsetup{labelformat=empty}
  \caption{Daily power consumption profiles (on day 7/9/2018) at ORD for HEAs with various BSED and MF values.
  Here, (\protect\solidorangeline) plots power requirements of single-aisle aircraft, (\protect\solidmidblueline) denotes the same for regional jets, (\protect\solidgreenline) is the sum of the above two profiles}
  \label{fig:Profile_ORD}
    %----------
    \subfloat[Regional Jets]{\includegraphics[width=0.4\textwidth]{figure/RJ_hist.jpg}}
    \subfloat[Single Aisle Aircraft]{\includegraphics[width=0.4\textwidth]{figure/SAs_hist.jpg}}
    \caption{Histograms and cumulative distribution functions (CDFs) of flight distances in ORD over 2018}
    \label{fig:Hist_CDF}
\end{figure}

Divide each day into 1440 one-minute intervals. Adding the charging requirements following the above procedure for all flights in a given 1-min interval yields the charging requirements for that interval. We plot a sample charging profile for ORD on 7/9/2018 with MF=12.5\%, but BSED of 500, 700 and 1000 Wh/kg in Figure \ref{fig:Profile_ORD}. Such profiles across all days in 2018 for each airport yield our results for annual energy and peak power requirements to power HEAs. 

We comment on an interesting observation from Figure \ref{fig:Profile_ORD}. Notice that as BSED increases, single-aisle aircraft begin to account for the lion's share of charging requirements. To explain this, we plot the frequency of different flight distances with the 300K+ regional jets and single aisle aircraft at ORD in 2018 in Figure \ref{fig:Hist_CDF}. 
The distance distribution of single-aisle aircraft is more right-skewed than that of regional jets. Indeed, the median distance of flights for single-aisle aircraft is 867 mi and for regional jets is 409 mi. As  larger travel distances are made possible with higher BSED, more single-aisle aircraft switch to become HEAs. These airplanes travel longer distances that typically require more energy than  regional jets traveling short distances. Thus, they constitute the bulk of the energy needs at higher BSED as shown in Figure \ref{fig:Profile_ORD}.

==> secmethod.tex <==
%!TEX root = main.tex

\subsection{Electricity Requirements with Uniform Charging Rate}
\label{sec:method}
The electricity demand of HEAs depends on the size of the domestic fleet that gets electrified, the type of flights being electrified, distances traveled and their charging schedules. We work with current flight schedules in this section and then generate a modified flight schedules to accommodate both charging requirements and passenger demands in section \ref{sec:SAmodel}.


we consider the most aggressive HEA uptake scenario where a commercial regional flight becomes an HEA if the flight distance is within its range. We divide each day into 1440 one-minute intervals. Adding the charging requirements of all flights in a given 1-min interval yields the charging requirements for that interval.
For each airport, we list all short-range domestic flights that had a dwell time longer than 15 minutes at that airport in 2018 from the BTS dataset. These airplanes are of two types--regional jets and narrow body aircraft. We then utilize the range capabilities of retrofit hybrid electric regional jets and narrow body aircraft from \cite{Wroblewski2019}. Thus, with a BSED-MF combination, we consider all flights with travel distances less than the maximum range achievable as HEAs. 


Assume that each HEA arrives at airport with zero charge in its battery. It then charges at a constant rate that is chosen so that the battery is charged up to the energy needs of the next flight leg by its departure time. Power required to serve such a flight leg is 
 $P =  E/T$,
where $E$ is the battery energy requirement and $T$ is the dwell time at airport (in minutes). Furthermore, the battery energy is given by
\begin{align}
    E = p  \times  d \times \gamma_0
    \label{eq:E.def}
\end{align}
required to travel $d$ miles with $p$ passengers. Here, $\gamma_0$ denotes the battery energy usage per passenger-mile. For each flight in the BTS database, we use the tail-number to identify the aircraft type from airplane manufacturer's websites, that in turn, yields the total number of seats on the plane. Throughout this analysis, we assume uniformly that 85\% of all seats are filled in each flight to estimate $p$. This load factor matches the yearly average estimates of the same by BTS (see \cite{BTSstatistics}).


The values of parameter $\gamma_0$ for HEAs are adopted from  \cite{Wroblewski2019}, assuming a battery-pack voltage of 128V. Their analysis accounts for battery energy consumed during taxi, takeoff, cruise, approach, and landing. To estimate $\gamma_0$ for a flight in the BTS dataset, we first identify whether it is a regional jet or a single-aisle (narrow-body) aircraft. For regional jets, we utilize $\gamma_0$ for ERJ-175  and for that of Boeing 737-700 for single-aisle aircraft. Battery sizes required for BSED below 700 Wh/kg and MF above 50\% are deemed impractical to use for any flight distance.

To illustrate the power demand requirements through an example, consider a single hybrid electric retrofit of Embraer ERJ 170-200 aircraft with tail number N178SY operating a 599 miles flight from SFO to SLC (Salt Lake City, UT) on 05/29/2018. 
N178SY arrives at SFO at 17:02 PM and leaves for SLC at 17:53 PM. For different MF and BSED configurations, we compute $E$ from \eqref{eq:E.def} and report in Table \ref{tab:OneFlight}. Dividing $E$ by 60 minutes yields the power requirements of N178SY from  17:02 to  17:53 PM on 05/29/2018. Also note that this example illustrate the case where a hybrid electric aircraft does not have the range ability to cover a flight mission of distance 599 miles under the setting of BSED being 500 Wh/kg and MF being 25\%.

\begin{table}[!ht]
\centering
\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{MF (\%)}  & \multicolumn{2}{c}{BSED (Wh/kg)} \\\cmidrule(lr{1em}){2-3}
 &500 & 700 \\
\midrule
12.5  & 1.23 MW & 1.22 MW \\
25  & / & 2.52 MW \\
\bottomrule
\end{tabular}
\caption {Power requirements of N178SY for flight from SFO to SLC.} 
\label{tab:OneFlight} 
\end{table}


% \begin{figure}[!h]
%     \centering
%     %---------
%     \subfloat[MF=12.5\%, BSED=500Wh/kg]{\includegraphics[width=0.33\textwidth]{elsarticle/figure/dailyORD500.jpg}\label{fig:Daily:1}}
%   \subfloat[MF=12.5\%, BSED=700Wh/kg]{\includegraphics[width=0.33\textwidth]{elsarticle/figure/dailyORD700.jpg}\label{fig:Daily:3}}
%   \subfloat[MF=12.5\%, BSED=1000Wh/kg]{\includegraphics[width=0.33\textwidth]{elsarticle/figure/dailyORD1000.jpg}\label{fig:Daily:7}}
%   %\captionsetup{labelformat=empty}
%   \caption{Daily power consumption profiles (on day 7/9/2018) at ORD for HEAs with various BSED and MF values.
%   Here, (\protect\solidorangeline) plots power requirements of single-aisle aircraft, (\protect\solidmidblueline) denotes the same for regional jets, (\protect\solidgreenline) is the sum of the above two profiles}
%   \label{fig:Profile_ORD}
%     %----------
%     \subfloat[Regional Jets]{\includegraphics[width=0.4\textwidth]{figure/RJ_hist.jpg}}
%     \subfloat[Single Aisle Aircraft]{\includegraphics[width=0.4\textwidth]{figure/SAs_hist.jpg}}
%     \caption{Histograms and cumulative distribution functions (CDFs) of flight distances in ORD over 2018}
%     \label{fig:Hist_CDF}
% \end{figure}

Divide each day into 1440 one-minute intervals. Adding the charging requirements following the above procedure for all flights in a given 1-min interval yields the charging requirements for that interval. Such profiles across all days in 2018 for each airport yield our results for annual energy and peak power requirements to power HEAs. 

We comment on an interesting observation. 
% from Figure \ref{fig:Profile_ORD}. 
Notice that as BSED increases, single-aisle aircraft begin to account for the lion's share of charging requirements. 
% To explain this, we plot the frequency of different flight distances with the 300K+ regional jets and single aisle aircraft at ORD in 2018 in Figure \ref{fig:Hist_CDF}. 
% The distance distribution of single-aisle aircraft is more right-skewed than that of regional jets. Indeed, the median distance of flights for single-aisle aircraft is 867 mi and for regional jets is 409 mi. 
As larger travel distances are made possible with higher BSED, more single-aisle aircraft switch to become HEAs. These airplanes travel longer distances that typically require more energy than  regional jets traveling short distances. 
% Thus, they constitute the bulk of the energy needs at higher BSED as shown in Figure \ref{fig:Profile_ORD}.

Several remarks on our analytic framework are in order.
First, a battery pack aboard an HEA cannot be charged at an arbitrary rate and must abide by the ratings of the battery and the charging equipment. We ignore such rate limitations in our calculations.  Second, arriving HEAs at an airport may have residual charge in their batteries that will impact charging requirements at the airport. We ignore such possibilities in our analysis. Third, we ignore the possibility that an HEA may need to charge enough to complete a round-trip journey from and to that airport if the destination location lacks necessary HEA charging infrastructure. Fourth, batteries often have efficiency losses that we ignore. Accounting for such losses will further increase the energy demands of HEAs. Relaxing one or more of these assumptions are relegated to future work.

%-----------
\subsection{The Optimization Problem for Smart Charging} \label{sec:smart}

Assume HEA operate under current flight schedule. We aim to flatten the aggregate charging profile over a pre-specified time horizon by managing charing demand of electrified aircraft that are hooked up to the grid. An any one moment during the time horizon, we coordinate the charging power delivered to each airplane that participates in charging events so that their cumulative charging requirement is minimal. We also ensure each aircraft has the capacity to commit its next flight. 

Recall that a day is divided into $T=1440$ one-minute intervals. Suppose, we consider the charging of $N$ HEAs, numbered $1, \ldots, N$. For aircraft $n=1,\ldots,N$, let $t_n^A$ and $t_n^D$, respectively, denote its arrival  and departure times at the airport gate. Define $E_n$ as its total energy needs for the next flight leg, calculated exactly as we did for naive charging. With $c_n(t)$ denoting the energy draw by HEA $n$ in period $t$, we formulate the smart charging problem as 
\begin{alignat}{2} \label{eq:smart}
\begin{aligned}
& {\text{minimize}} \ \ && \sum_{t=1}^{T}\left(\sum_{n=1}^{N} c_{n}(t)\right)^{2}, \\
& \text {such that} \ \ && 
 \sum_{t =1}^T c_{n}(t) = E_{n}, \ c_{n}(t)=0 \text{ for } t \notin\left[t_n^A, t_n^D\right], \ n=1,\ldots,N, \\
 &&& 
\underline{c}_{n} \leq c_{n} \leq \overline{c}_{n}
\end{aligned}
\end{alignat}
over $c_n(t)$ for $n=1,\ldots,N$ and $t=1,\ldots,T$. The two constraints encode the requirement that HEA $n$ must fulfill its charging obligations over the time it is parked at the airport gate and that batteries, power electronics, and associated cables may impose constraints on the power level that can be attained. Constraints on C-rate, as described in \ref{sec:analysis}, are encoded in $\overline{c}_{n}$. The quadratic objective function is such that it seeks to flatten the charging profile within the constraints described. The quadratic program is solved using python with a Gurobi solver to generate the results in Table \ref{tab:airports} and Figures \ref{fig:C_const} and \ref{fig:IAD_30min}.






